Country-scale Exploratory Analysis of Call Detail Records through the Lens of Data Grid Models

Call Detail Records (CDRs) are data recorded by telecommunications companies, consisting of basic informations related to several dimensions of the calls made through the network: the source, destination, date and time of calls. CDRs data analysis has received much attention in the recent years since it might reveal valuable information about human behavior. It has shown high added value in many application domains like e.g., communities analysis or network planning. In this paper, we suggest a generic methodology for summarizing information contained in CDRs data. The method is based on a parameter-free estimation of the joint distribution of the variables that describe the calls. We also suggest several well-founded criteria that allows one to browse the summary at various granularities and to explore the summary by means of insightful visualizations. The method handles network graph data, temporal sequence data as well as user mobility data stemming from original CDRs data. We show the relevance of our methodology for various case studies on real-world CDRs data from Ivory Coast.

==> conclusion.tex <==
\section{Conclusion \& discussion}
\label{sec:conclusion}
%
We have suggested a method for coclustering and exploratory analysis of categorical time series (or temporal event sequences) based on three-dimensional data grid models. The sequence identifiers are grouped into clusters, the time dimension is discretized into intervals and the events are also grouped into clusters -- the whole forming a 3D-grid. The optimal grid (the most probable a posteriori in Bayesian terms) is obtained with an user parameter-free procedure. To exploit the resulting grid, we have suggested \textit{(i)} a dissimilarity index between clusters to select the wanted granularity of the grid while controlling the information loss; \textit{(ii)}, a criterion, namely the typicality, to rank and identify representative values in a cluster; \textit{(iii)} two other criteria stemming from Mutual Information to characterize, interpret and visualize the found clusters. Our insightful findings have been illustrated on both synthetic and real-world data sets.
%Nous avons proposé une méthode de clustering et d'analyse de séquences temporelles basée sur les modèles en grille. Les identifiants de séquence sont groupés en clusters, ainsi que les évènements, et la dimension temporelle est discrétisée en intervalles -- le tout forme ainsi une grille tridimensionnelle (ou tri-clustering). Obtenir la grille optimale (au sens Bayésien) ne nécessite aucun paramétrage utilisateur. Pour exploiter la grille, nous avons proposé \textit{(i)} une mesure de dissimilarité entre clusters afin de sélectionner le grain de la grille tout en contrôlant la perte d'information, \textit{(ii)}, un critère (la typicité) pour identifier les valeurs les plus représentatives d'un cluster, \textit{(iii)} ainsi que deux critères basés sur l'information mutuelle pour caractériser, interpréter et visualiser les clusters trouvés. Nos différentes propositions ont été validées sur des données simulées ainsi que sur des données réelles issues de \textsc{dblp}. Notons qu'une étude du comportement asymptotique des indicateurs proposés a été réalisée et qu'une étude complète des trajectoires antenne-antenne d'utilisateurs du mobile -- que l'on peut voir comme des séquences d'évènements -- a été menée à l'échelle d'un pays (voir \cite{Gui13}).

==> exploitation.tex <==
%exploitation.tex
\section{Exploiting the grid}
\label{sec:exploitation}
%

In some real-world large-scale case studies, the grid resulting from the optimization procedure is made of several hundreds of clusters of cats ids (or intervals and/or clusters of events), i.e. millions of cells, which makes the results difficult to exploit and interpret.

\noindent \textbf{Dissimilarity index and grid structure simplification.}
%
We suggest a simplification method of the grid structure that iteratively merge clusters or adjacent intervals -- choosing the merge generating the least degradation of the grid quality. To this end, we introduce a dissimilarity index between clusters or intervals which characterize the impact of the merge on the $cost$ criterion.

\begin{definition}[Dissimilarity index]
Let $c_{.1}$ and $c_{.2}$ be two parts of a dimension partition of a grid model $M$ (i.e. two clusters of sequence ids or events or two adjacent intervals). Let $M_{c_{.1}\cup c_{.2}}$ be the grid after merging $c_{.1}$ and $c_{.2}$. The dissimilarity $\Delta(c_{.1},c_{.2})$ between the two parts $c_{.1}$ and $c_{.2}$ is defined as the difference of $cost$ before and after the merge:
%
\begin{align}
\Delta(c_{.1},c_{.2}) = cost(M_{c_{.1}\cup c_{.2}}) - cost(M) \nonumber
\end{align}
\end{definition}
%

When merging clusters that minimize $\Delta$, we obtain the sub-optimal grid $M'$ (with a coarser grain, i.e. simplified) with minimal $cost$ degradation, thus with minimal information loss w.r.t. the grid $M$ before merging. The information rate of the grid $M'$ is defined as follows:
%
\begin{align}
IR(M') = (cost(M')-cost(\mathcal{M_{\emptyset}})) / (cost(M^*) - cost(M_{\emptyset})) \nonumber
\end{align}
%

where $M_{\emptyset}$ is the null model (the grid where no dimension is partitioned). Performing the best merges w.r.t. $\Delta$ iteratively over the three dimensions without distinction, starting from $M^{\ast}$ until $M_{\emptyset}$, three agglomerative hierarchies are built and the end-user can stop at the chosen granularity that is necessary for the analysis while controlling either the number of clusters/cells or the information rate kept in the model.

\noindent \textbf{Typicality for ranking categorical values in a cluster.} When the chosen granularity is reached through agglomerative hierarchy, the number of clusters per categorical dimension (cats ids or events) decreases and mechanically the number of values per cluster increases. It could be useful to focus on the most representative values (cats ids or events) among thousands of values of a cluster. In order to rank values in a cluster, we define the typicality of a value as follows:
%
\begin{definition}[Typicality of a value in a cluster]
For a value $v$ in a cluster $c$ of the partition $X^M$ of dimension $X$ given the grid model $M$, the typicality of $v$ is defined as:
%
\begin{align}
\tau (v,c) = \frac{1}{1-P_{X^M}(c)} \sum_{c_j\in X^M\atop c_j\neq c} P_{X^M}(c_j)(cost(M|c\setminus v,c_j\cup v)-cost(M)) \nonumber
\end{align}
%
where $P_{X^M}(c)$ is the probability of having a point with its value in cluster $c$, $c\setminus v$ is the cluster $c$ from which we have removed value $v$, $c_j\cup v$ is the cluster $c_j$ to which we add value $v$ and $M|c\setminus v,c_j\cup v$ the grid model $M$ after the aforementioned modifications.
\end{definition}
%
Intuitively, the typicality evaluates the average impact in terms of $cost$ on the grid model quality of removing a value $v$ from its cluster $c$ and reassigning it to another cluster $c_j\neq c$. Thus, a value $v$ is representative (say typical) of a cluster $c$ if $v$ is ``close'' to $c$ and ``different in average'' from other clusters $c_j\neq c$.\\
%
In~\cite{Gui13} chapter 4, asymptotic behaviors (when $N\to \infty$) of the dissimilarity index $\Delta$ and typicality $\tau$ have been studied. It was found and demonstrated that \textit{(i)} the dissimilarity $\Delta(c_{.1},c_{.2})$ can be interpreted as the Jensen-Shannon divergence between probability laws $P_{X_1^M|c_{.1}}$ and $P_{X_1^M|c_{.2}}$ of partitioned variable $X_1^M$ conditionally to clusters $c_{.1}$ and $c_{.2}$; \textit{(ii)} the typicality $\tau (v,c)$ of a value $v$ can be interpreted as a sum of Kullback-Liebler divergences. Both asymptotic behaviors confirm the intuitions  behind the two criteria given above.% Tedious proofs~\cite{Gui13} are omitted to fit with space limitations.\\
%

\noindent \textbf{Insightful visualizations with Mutual Information and Contrast.}
%
It is common to visualize 2D coclustering results using 2D frequency matrix or heat map. For 3D coclustering, it is useful to select a dimension of interest (in our case, sequence ids $S$) and then we are able to visualize the frequency matrix of the two other dimensions ($T$ and $E$) given a cluster $c$ of $S$. We also suggest two other insightful measures for coclusters to be visualized, namely, the Contribution to Mutual Information (CMI) and the Contrast -- providing additional valuable visual information inaccessible with only frequency representation. Notice that the contributed visualizations are also valid whatever the dimension of interest.

\begin{definition}[Mutual Information and Contribution]
For a cluster of cats ids $c_{i_S}$, the mutual information between two partitioned variables $T^{\pi_M}$ and $E^{\pi_M}$ (from the partition $\pi_M$ of time and event variables induced by the grid model $M$) is defined as:
%
\begin{align}
MI(T^{\pi_M};E^{\pi_M})=\sum_{i_1=1}^{i_1=k_{T}}\sum_{i_2=1}^{i_2=k_{E}}MI_{i_1i_2} \nonumber \\
\text{where} \quad MI_{i_1i_2}=p(c_{i_1i_2})\log \frac{p(c_{i_1i_2})}{p(c_{i_1})p(c_{i_2})}
\end{align}
%
where $MI_{i_1i_2}$ represent the contribution of cell $c_{i_1i_2}$ to the mutual information.
\end{definition}
%
Thus, if $MI_{i_1i_2} > 0$ then $p(c_{i_1i_2}) > p(c_{i_1})p(c_{i_2})$ and we observe an excess of interaction between $c_{i_1}$ and $c_{i_2}$ located in cell $c_{i_1i_2}$ defined by time interval $T_{i_1}$ and group of events $E_{i_2}$. Conversely, if $MI_{i_1i_2} < 0$, then $p(c_{i_1i_2}) < p(c_{i_1})p(c_{i_2})$, and we observe a deficit of interactions in cell $c_{i_1i_2}$. Finally, if $MI_{i_1i_2} = 0$, then either $p(c_{i_1i_2})=0$ in which case the contribution to MI is null and there is no interaction or $p(c_{i_1i_2}) = p(c_{i_1})p(c_{i_2})$ and the quantity of interactions in $c_{i_1i_2}$ is that expected in case of independence between the partitioned variables.


%\textit{Visualisation de l'information mutuelle.} Pour un cluster de séquences $c_{i_S}$, l'information mutuelle entre les variables $T^{\pi_M}$ et $E^{\pi_M}$ issues du partitionnement $\pi_M$ des variables temps et évènement généré par le modèle de grille $M$, est défini comme suit:
%%
%\begin{align}
%MI(T^{\pi_M};E^{\pi_M})=\sum_{i_1=1}^{i_1=k_{T}}\sum_{i_2=1}^{i_2=k_{E}}MI_{i_1i_2} \quad \text{où} \quad MI_{i_1i_2}=p(c_{i_1i_2})\log \frac{p(c_{i_1i_2})}{p(c_{i_1.})p(c_{.i_2})}
%\end{align}
%
%Ainsi, les $MI_{i_1i_2}$ représentent la contribution de la cellule $c_{i_1i_2}$ à l'information mutuelle. Si $MI_{i_1i_2} > 0$, alors $p(c_{i_1i_2}) > p(c_{i_1.})p(c_{.i_2})$, et on observe un excès d'interactions entre $c_{i_1.}$ et $c_{.i_2}$ localisé dans la cellule $c_{i_1i_2}$ définie par l'intervalle $T_{i_1}$ et le groupe d'évènements $E_{i_2}$. Inversement, si $MI_{i_1i_2} < 0$, alors $p(c_{i_1i_2}) < p(c_{i_1.})p(c_{.i_2})$, et on observe un déficit d'interactions dans la cellule $c_{i_1i_2}$. Enfin, si $MI_{i_1i_2} = 0$, alors soit $p(c_{i_1i_2})=0$ auquel cas la contribution à l'information mutuelle est nulle et il n'y a pas d'interactions; soit $p(c_{i_1i_2}) = p(c_{i_1.})p(c_{.i_2})$ et la quantité d'interactions dans $c_{i_1i_2}$ est celle attendue en cas d'indépendance des partitions.

\begin{definition}[Contrast]
%For the couple of partitioned variables to be visualized ($T^{\pi_M}$, $E^{\pi_M}$), the contrast between a context, i.e., a cluster of cats ids $c_{i_S}$, and the union of other clusters of cats ids $\{c_i\}_{i\neq i_S}$ is defined as:
%
The contrast between the two partitioned variables to be visualized $(T^{\pi_M},E^{\pi_M})$ considered jointly and $S^{\pi_M}$ is defined as:
\begin{align}
Contrast((T^{\pi_M},E^{\pi_M}),S^{\pi_M}) = \sum_{i_S=1}^{i_S=k_{S}}\sum_{i_1=1}^{i_1=k_{T}}\sum_{i_2=1}^{i_2=k_{E}}MI_{i_Si_1i_2} \nonumber \\
\text{where} \quad MI_{i_Si_1i_2}=p(c_{i_Si_1i_2})\log \frac{p(c_{i_Si_1i_2})}{p(c_{i_1i_2})p(c_{i_S})} \nonumber
\end{align}
%
\end{definition}
%
Again, the sign of $MI_{i_Si_1i_2}$ values explains what is contrasting in $c_{i_S}$ w.r.t. the set of all sequence ids from the view $(T^{\pi_M},E^{\pi_M})$. Positive and negative values both highlight the cells that characterize $c_{i_S}$ w.r.t. the set of all sequence ids; the former says that an excess of interaction is located in cell $c_{i_1i_2i_S}$, the latter highlights a deficit of interaction (a negative contrast); and $MI_{i_1i_2i_S}=0$ (or nearly) indicates no significant contrast.

While the visualization of cells' CMI highlight valuable information that is local to a cluster of cats, the contrast is a global scope visualization. Both CMI and contrast bring complementary insights to exploit the summary provided by the grid. In our experiments, we show the added-value of those visualizations on both synthetic and real data sets.

%\noindent \textit{Visualisation du contraste.} Pour le couple de variables partitionnées à visualiser ($T^{\pi_M}$, $E^{\pi_M}$), le contraste entre un contexte, i.e., un cluster de séquences $c_{i_S}$ et le reste des clusters de séquences $\{c_i\}_{i\neq i_S}$ est défini comme suit:
%%
%\begin{align}
%Contraste(c_{i_S}) = MI((T^{\pi_M},E^{\pi_M});c_{i_S})=\sum_{i_1=1}^{i_1=k_{T}}\sum_{i_2=1}^{i_2=k_{E}}MI_{i_1i_2;i_S} \\
%\text{où} \quad MI_{i_1i_2;i_S}=p(c_{i_1i_2i_S})\log \frac{p(c_{i_1i_2i_S})}{p(c_{i_1i_2.})p(c_{..i_S})} \nonumber
%\end{align}
%% $$\text{où} \quad MI_{i_1i_2;i_S}=p(c_{i_1i_2i_S})\log \frac{p(c_{i_1i_2i_S})}{p(c_{i_1i_2.})p(c_{..i_S})}$$
%%
%Comme précédemment, le signe des $MI_{i_1i_2;i_S}$ qualifiera le contraste entre $c_{i_S}$ et le reste des données (i.e., les clusters de séquences $\{c_i\}_{i\neq i_S}$). Les valeurs de $MI_{i_1i_2;i_S}$ sont rapportées dans les figures ~\ref{fig:2cats_vis}$M_1$(c) et ~\ref{fig:2cats_vis}$M_2$(c). Prenons le cluster de séquences de $c_{M_1}$. Les cellules blanches indiquent qu'il n'y a pas de contraste à cet endroit entre $c_{M_1}$ et le reste des données (ici, $c_{M_2}$): par exemple la cellule $([0;100],\{g,h,i\})$, malgré le bruit, n'est pas caractéristique de $c_{M_1}$; en effet, la probabilité du groupe d'évènements $\{g,h,i\})$ dans l'intervalle de temps $([0;100]$ n'est pas significativement différent selon qu'on se trouve dans $c_{M_1}$ ou $c_{M_2}$. De même la cellule $([401;500],\{d,e,f\})$ présente un contraste nul puisqu'elle est commune aux deux motifs sous-jacents. Les cellules rouges indiquent ce qui caractérise $c_{M_1}$ par rapport à $c_{M_2}$: dans ces cellules, la probabilité de points est bien supérieure pour $c_{M_1}$ que pour $c_{M_2}$. Les cellules bleues indiquent un contraste négatif: la probabilité de points y est plus faible pour $c_{M_1}$ que pour $c_{M_2}$.


%\noindent \textbf{Typicité d'une valeur d'un cluster.} Pour une valeur $v_i$ d'un cluster $c$ de la partition $X^M$ de la variable $X$ selon le modèle de grille $M$, la typicité est définie par:
%%
%\begin{align}
%\tau (v_i) = \frac{1}{1-P_{X^M}(c)} \sum_{c_j\in X^M\atop c_j\neq c} P_{X^M}(c_j)(cost(M|c\setminus v,c_j\cup v)-cost(M))
%\end{align}
%%
%où $P_{X^M}(c)$ est la probabilité d'avoir un point avec une valeur du cluster $c$, $c\setminus v$ est le cluster $c$ duquel on a retiré la valeur $v$, $c_j\cup v$ est le cluster $c_j$ auquel on a rajouté la valeur $v$ et $M|c\setminus v,c_j\cup v$ le modèle de grille $M$ qui a subi les modifications précitées. Intuitivement, une valeur $v_i$ est représentative d'un cluster $c$ et dite typique, si elle est proche de $c$ et très différente (en moyenne) des autres clusters $c_j\neq c$. Aussi, pour un cluster d'auteurs, les auteurs qui ont peu publié (1 ou 2 fois, voir figure~\ref{fig:distrib_auteur_publi}) sont souvent moins typiques que ceux qui sont les plus prolifiques, puisque si on les déplace vers un autre cluster, la différence de $cost$ (dans la formule de la typicité) sera faible.
